Markov $\alpha$-Potential Games

We propose a new framework of Markov $\alpha$-potential games to study Markov games. We show that any Markov game with finite-state and finite-action is a Markov $\alpha$-potential game, and establish the existence of an associated $\alpha$-potential function. Any optimizer of an $\alpha$-potential function is shown to be an $\alpha$-stationary Nash equilibrium. We study two important classes of practically significant Markov games, Markov congestion games and the perturbed Markov team games, via the framework of Markov $\alpha$-potential games, with explicit characterization of an upper bound for $\alpha$ and its relation to game parameters. Additionally, we provide a semi-infinite linear programming based formulation to obtain an upper bound for $\alpha$ for any Markov game. Furthermore, we study two equilibrium approximation algorithms, namely the projected gradient-ascent algorithm and the sequential maximum improvement algorithm, along with their Nash regret analysis, and corroborate the results with numerical experiments.

==> Sections/NearMPG.tex <==
  This section introduces the notion of Markov $\mnpg$-potential games, and  presents the properties of stationary Nash equilibrium in this game framework.  
    To begin with, recall the  definition of Markov potential games proposed by \citet{leonardos2021global}. 
    \begin{definition}[Markov potential games (\citet{leonardos2021global})]\label{def: PotentialGame} A Markov game \(\game\) is a Markov potential game if there exists a potential function 
  %  \(\potential: S \times \Pi\ra \mathbb{R}\) 
   \(\potential \in \mathcal{F}\) 
    such that for any \(i \in \playerSet\),  $s\in S$,  \(\policy_i,\policy_i'\in \Pi_i\), and  \(\policy_{-i}\in \Pi_{-i}\),
\begin{align}\label{eq:potential_function}
        \Phi(s, \policy_i',\policy_{-i}) -  \Phi(s, \policy_i,\policy_{-i})= \vFunc_i(s, \policy_i',\policy_{-i}) -  \vFunc_i(s, \policy_i,\policy_{-i}). %~ \forall i \in \playerSet, ~ \forall \policy_i, \policy_i^{'} \in \Pi_i, \text{ and } \forall \policy_{-i}\in \Pi_{-i}.
    \end{align}
  %   {\color{blue} Let $\Phi(\rho, \pi) := \mathbb{E}_{s\sim \rho}[\Phi(s, \pi)]$ be the expected potential function over a state distribution $\rho \in \Delta(S)$.}
    \end{definition}
That is, a game is an MPG if there exists a potential function such that when a player unilaterally deviates from her policy,  the change of the potential function is equal to the change of her expected payoff. 
As pointed out earlier, a key shortcoming of the MPG framework is the difficulty (\citet{narasimha2022multi}) to check the existence or to compute \(\Phi\), thus limiting the scope of its real-world applications.

Instead, we propose to relax the equality in \eqref{eq:potential_function} to allow the difference between the change of any player's payoff from unilateral deviation and the change of the potential function to be bounded by some $\mnpg\geq 0$, under the notion of \emph{Markov \(\mnpg\)-potential games}. More precisely,

% \begin{definition}[Markov \(\mnpg\)-potential game]
%     A Markov game $\mathcal{G}$ is a Markov $\mnpg$-potential game for some $\mnpg\geq0$, if there exists a state-dependent potential function $\Phi: S \times \Pi \rightarrow \mathbb{R}$ such that for every $s \in S,$
% \begin{equation}\label{eqn: def eps MPG}
%     |\left(\Phi\left(s, \pi_i^{\prime}, \pi_{-i}\right)-\Phi\left(s, \pi_i, \pi_{-i}\right)\right) - \left(V_i\left(s, \pi_i^{\prime}, \pi_{-i}\right)-V_i\left(s, \pi_i, \pi_{-i}\right)\right)|\leq \mnpg,
% \end{equation}
% for any $i \in I$, any $\pi_i, \pi_i^{\prime} \in \Pi_i$, and any $\pi_{-i} \in \Pi_{-i}$. We refer \(\Phi\) as a \(\mnpg\)-potential function.
% \end{definition}


{
\begin{definition}[Markov $\alpha$-potential game]\label{def: eps MPG} A Markov game $\mathcal{G}$ is a Markov $\alpha$-potential game, if there exists  some $\alpha \geq 0$ such that
    \begin{equation}\label{eqn: def eps MPG}
             \alpha := \inf_{\Psi\in \mathcal{F}} 
             \sup_{
             s\in S, i\in I, 
                \pi_i,\pi'_i \in \Pi_i, 
                \pi_{-i} \in \Pi_{-i}}
            \left| \Psi\left(s, \pi_i^{\prime}, \pi_{-i}\right)-\Psi\left(s, \pi_i, \pi_{-i}\right) - \left(V_i\left(s, \pi_i^{\prime}, \pi_{-i}\right)-V_i\left(s, \pi_i, \pi_{-i}\right)\right) \right|.
    \end{equation}
\end{definition} 
Moreover, if there exists some  $\Phi \in \mathcal{F}$ such that
$$
\alpha = {\sup_{s\in S, i\in I,
                 \pi_i,\pi'_i \in \Pi_i, 
                 \pi_{-i} \in \Pi_{-i}} }
             \left| \Phi\left(s, \pi_i^{\prime}, \pi_{-i}\right)-\Phi\left(s, \pi_i, \pi_{-i}\right) - \left(V_i\left(s, \pi_i^{\prime}, \pi_{-i}\right)-V_i\left(s, \pi_i, \pi_{-i}\right)\right) \right|, 
$$
then we can call $\Phi$ the associated  $\alpha$-potential function.
\begin{remark}\label{rem:definition}
    
Throughout the paper, our analysis does not assume {\it a priori} the existence of an $\alpha$-potential function $\Phi$. Instead, if one can find a feasible solution $\Psi \in \mathcal{F}$ to \eqref{eqn: def eps MPG} that yields an upper bound $\bar{\alpha}$ for $\alpha$, i.e., $\bar{\alpha} =\sup_{s\in S, i\in I,
                 \pi_i,\pi'_i \in \Pi_i, 
                 \pi_{-i} \in \Pi_{-i}} 
             | \Psi\left(s, \pi_i^{\prime}, \pi_{-i}\right)-\Psi\left(s, \pi_i, \pi_{-i}\right) - \left(V_i\left(s, \pi_i^{\prime}, \pi_{-i}\right)-V_i\left(s, \pi_i, \pi_{-i}\right)\right) |$, 
then one can infer that $\mathcal{G}$ is a Markov $\alpha$-potential game with $\alpha \in [0, \bar{\alpha}]$. 

In Section \ref{ssec: FindClosestMPG}, we will present an optimization-based approach for determining the upper bound of $\mnpg$ for general Markov games, assuming certain structure for feasible solutions $\Psi$ as defined in \eqref{eqn: F tilde}. In the special case when (the upper bound of) the parameter \(\mnpg\) is $0$, 
a Markov \(\mnpg\)-potential game is an MPG.
\end{remark}
}


% {\color{blue} 
% Note that here we do not impose any conditions to 
% 1. (we do not impose any conditions to $\mathcal{F}$ to make sure there exists a $\Phi$; )

% 2. (because if we can find a feasible solution $\Psi \in \mathcal{F}$ which yields an upper bound $\alpha'$ of $\alpha$, i.e., $\alpha' = \max|\Psi - \Psi' - V_i + V_i'|$, then one can conclude that $\mathcal{G}$ is a Markov $\alpha$-pg with $\alpha \leq \alpha'$.

% 3. (In Section \ref{ssec: FindClosestMPG}, we will present an optimization-based characterization to find the upper bound of $\mnpg$ for general Markov games when assuming $\Psi$ follows certain structure (cf. \eqref{eqn: F tilde})). }

%Note that in order to show a given Markov game is a  Markov \(\mnpg\)-potential game, it is sufficient to find a feasible solution $\Psi \in \mathcal{F}$ which yields an upper bound of $\alpha$. Our goal is not to find the exact $\alpha$-potential function $\Phi$. Instead, we aim to construct a feasible solution to \eqref{eqn: def eps MPG}  }



% [old version:] In the special case when the parameter \(\mnpg=0\), 
% a Markov \(\mnpg\)-potential game is an MPG.
% Note that in order to show a given Markov game is a  Markov \(\mnpg\)-potential game, it is sufficient to derive an upper bound of $\alpha$.   In Section \ref{ssec: FindClosestMPG}, we will present an optimization-based characterization to find the upper bound of $\mnpg$ for general Markov games. 
%  \todo[inline]{
% Argument to replace inf with min in definition of alpha: Note that as we assumed that \(\Psi\) is continuous function then the function
%  \begin{align*}
%    f(\Psi,\pi,\pi') =  \max_{s\in S, i\in I} 
%              \left| \Psi\left(s, \pi_i^{\prime}, \pi_{-i}\right)-\Psi\left(s, \pi_i, \pi_{-i}\right) - \left(V_i\left(s, \pi_i^{\prime}, \pi_{-i}\right)-V_i\left(s, \pi_i, \pi_{-i}\right)\right) \right| 
%  \end{align*}
%  is continuous under the standard topology induced by sup-norm on \(\mathcal{F}\times \Pi\times \Pi\). Then by Berge's maximum theorem we are guaranteed that the functiong \(g(\Psi) = \max_{\pi,\pi'}f(\Psi, \pi,\pi')\) is continuous. Moreover we know that \(\mathcal{F}\) is relatively compact in set of continuous functions over a compact set. Therefore by extreme value theorem \cite{rudin1953principles}, we can replace \(inf_{\Psi}\) with \(min_{\Psi}\)
%  % we would need to ensure that the set \(\mathcal{F}\) is compact with respect to appropriate topology on function space. This for example can be true if we impose that the set \(\mathcal{F}\) is equicontinuous and pointwise bounded. 
%  }
% Second, the parameter \(\alpha\) is not a \emph{design choice} but rather a structural characteristic of the underlying Markov game \(\game\) which characterizes its ``distance'' with a Markov potential game.
 % }
\subsection{Examples of Markov $\mnpg$-potential game}\label{ssec: ExamplesNearMPG}

 There exist two important and well-known classes of games that are not Markov potential games. We will demonstrate that these  games can be analyzed in the framework of Markov $\mnpg$-potential games, with  explicit expressions for the upper bounds of $\mnpg$.
%with explicit construction of their respective \(\mnpg\)-potential functions.

\paragraph{Markov congestion game (MCG).}  The Markov congestion game $\game_{\textsf{mcg}}$ is a dynamic counterpart of the static congestion game introduced by \citet{monderer1996potential}, with a finite number of players using a finite set of resources. Each stage of $\game_{\textsf{mcg}}$ is a static congestion game with a state-dependent reward function for each resource, and the state transition depends on players' aggregated usage of each resource. 
Specifically, denote the finite set of resources in the one-stage congestion game as $E$. The action $a_i \in A_i \subseteq 2^{E}$ of each player $i \in I$ is the set of resources chosen by player $i$. Here the action set $A_i$ is the set of all resource combinations that are feasible for player $i$. The total usage demand of all players is $1$, and each player's demand is assumed to be $1/|I|$, for  simplicity and without loss of generality. Given an action profile $a=(a_i)_{i \in I}$, the aggregated usage demand of each resource $e \in E$ is given by 
\begin{align}\label{eq:w}
w_e(a) =  \frac{1}{|I|}\sum_{i\in I}\mathbbm{1}(e \in a_i) .
\end{align}
In each state $s$, the reward for using resource $e$ is denoted as $(1/|I|)\cdot c_e(s, w_e(a))$. Thus, the one-stage payoff for player \(i\in I\) in state \(s\in S\) given the joint action profile \(a\in A\) is  \(u_i(s,a) = \frac{1}{|I|}\sum_{e\in a_i}c_e(s, w_e(a))\).  The state transition probability, denoted as $P(s'|s,w)$, depends on the aggregate usage vector $w=(w_e)_{e \in E}$ induced by players' action profile as in \eqref{eq:w}.  The set of all feasible aggregate usage demand is denoted by \(W\).
The next proposition shows that \(\game_{\textsf{mcg}}\) is a Markov \(\mnpg\)-potential game under a suitable Lipschitz condition for the state transition probability. 
\begin{proposition}\label{prop:mcg}
If there exists some $\zeta>0$ such that  
\begin{align*}
    |P(s'|s,w)-P(s'|s,w')| \leq \zeta  \|w-w'\|_{1}, \quad \forall \ s, s'\in S, w, w'\in W,
\end{align*}
then the
    congestion game \(\game_\textsf{mcg}\) is a Markov \(\mnpg\)-potential game with 
   {\(
        \mnpg \leq \frac{2\zeta |S| \delta|E|\sup_{s,\pi}\Psi(s,\pi)}{|I|(1-\delta)}
    \)}
and
\begin{align}\label{eq:potential}
\Psi(\mu, \pi)=\frac{1}{|I|}\avg_{\mu,\pi}\Bigg[\sum_{k=0}^{\infty}\delta^k \bigg(\sum_{e\in E}\sum_{j=1}^{w_e^k |I|}c_e\Big(s^k, \frac{j}{|I|}\Big)\bigg)\Bigg],
\end{align}
where \(s^0\sim \initDist\), the aggregate usage vector $w^k = (w_e^k)_{e \in E}$ is induced by \(a^k\sim \policy(s^k)\), and \(s^k\sim \transition(\cdot|s^{k-1},w^{k-1})\).
\end{proposition}
Proof of Proposition \ref{prop:mcg} is provided in Appendix \ref{ssec: ProofMCG}.

Note that the expression in \eqref{eq:potential} is the expected value of the summation of each stage's static potential function. There are two key steps for the derivation:
% This is not hard to derive:
first, each static congestion game at stage $k$ is a potential game with the corresponding potential function as $1/|I|\sum_{e\in E}\sum_{j=1}^{w_e^k |I|}c_e\left(s^k, j/|I|\right)$;  second, as established in Lemma \ref{lem: CongestionGameTransitionDifference}, 
% according to  Lemma \ref{lem: CongestionGameTransitionDifference},
the change of state transition probability induced by a single player's policy deviation decreases as the number of players increases. 
Furthermore, the upper bound of $\mnpg$ scales linearly with respect to the Lipschitz constant $\zeta$, the size of state space $|S|$, resource set $|E|$, and decreases as $|I|$ increases. 
  As $|I| \to \infty$, this  \(\game_{\textsf{mcg}}\) becomes an MPG. 



          



\paragraph{Perturbed Markov team game (PMTG).}
Consider a Markov game \(\pertCommonGame=\langle S, (A_i)_{i\in I}, (u_i)_{i\in I}, P, \delta \rangle \), where the payoff function for each player \(i\in I\) can be decomposed as \(u_i(s,a) = r(s,a) + \xi_i(s,a)\). Here  $r(s,a)$ represents the common interest for  the team, and  \(\xi_i(s,a)\) represents each player $i$'s heterogeneous preference such  that \(\|\xi_i(\cdot)\|_{\infty}\leq \kappa\), where $\kappa \ge 0$  measures each player's deviation from the team's common interest. As $\kappa \to 0$, \(\game_{\textsf{pmtg}}\) becomes an  Markov team game, which is an MPG (\citet{leonardos2021global}). 
The next proposition shows that a \(\game_{\textsf{pmtg}}\) is a Markov \(\mnpg\)-potential game, and the upper bound of $\mnpg$ decreases in the magnitude of payoff perturbation $\kappa$. 
\begin{proposition}\label{prop: PerturbedMarkovTeamGame}
    A perturbed Markov team game \(\pertCommonGame\) is a Markov \(\mnpg\)-potential game with 
{\(
        \mnpg \in [0, \frac{2\kappa}{(1-\delta)^2}].
    \)}
%     and the corresponding \(\mnpg\)-potential function \(
% \Phi(\mu, \pi)=\avg\left[\sum_{k=0}^{\infty}\delta^k r(s^k, a^k)\right],
% \)
% where \(s^0\sim \initDist\), \(a^k\sim \policy(s^k)\), and \(s^k\sim \transition(\cdot|s^{k-1},w^{k-1})\).
\end{proposition}
Proof of Proposition \ref{prop: PerturbedMarkovTeamGame} is provided in Appendix \ref{ssec: ProofPMTG}. 


\subsection{Finding (an upper bound of) $\mnpg$}\label{ssec: FindClosestMPG}
\input{Sections/NearestPotentialGame}

\input{Sections/PropertiesOfNearMPG}

==> Sections/PropertiesOfNearMPG.tex <==

 
\begin{comment}
{\subsection{Properties of Markov  $\mnpg$-potential game}  \color{gray}
%\xinyu{The following parts have been included before}
To analyze the Markov  $\mnpg$-potential games, we adopt the criterion of stationary Nash equilibrium.   
First, recall   \begin{definition}[Stationary Nash equilibrium]
   A policy profile \(\policyNash  = (\pi_i^*, \pi_{-i}^*)\) is a stationary Nash equilibrium of a Markov game $\game$ if for any \(i\in \playerSet\), any \(\policy_i\in\Pi_i\), and any \(\initDist\in\Delta(\stateSet)\),
    \(
        \vFunc_i(\mu, \policyNash_i,\policyNash_{-i}) \geq \vFunc_i(\mu, \policy_i,\policyNash_{-i}).
    \)
    \end{definition}
That is, a stationary policy profile is a stationary Nash equilibrium of the game $\game$ if each player's policy maximizes her expected total payoff given other players' equilibrium policy. 
A stationary Nash equilibrium always exists in any Markov game with finite states and actions (\citet{fudenberg1998theory}).
    \begin{definition}[$\epsilon$-Stationary Nash equilibrium]\label{def: eps NE}
    For any $\epsilon \geq 0$, a policy profile \(\policyNash  = (\pi_i^*, \pi_{-i}^*)\) is an $\epsilon$-stationary Nash equilibrium of a Markov game $\game$ if for any \(i\in \playerSet\), any \(\policy_i\in\Pi_i\), and any \(\initDist\in\Delta(\stateSet)\),
    \(
        \vFunc_i(\mu, \policyNash_i,\policyNash_{-i}) \geq \vFunc_i(\mu, \policy_i,\policyNash_{-i}) -\epsilon.
    \)
    \end{definition} 
 Clearly, as $\epsilon \to 0$, an $\epsilon$-stationary Nash equilibrium becomes a stationary Nash equilibrium.
Now we can establish the equilibrium properties of Markov $\mnpg$-potential game.
 





\begin{proposition}\label{prop:approximate_eq}%[Equilibrium properties of Markov near potential %games]\label{prop: RelationBWEpsEq} 
Consider a Markov \(\mnpg\)-potential game $\game$ with an {$\mnpg$-potential function} \(\Phi\). For any $\epsilon > 0$, a policy profile \(\pi^\ast\in \Pi\) is an $(\mnpg + \epsilon)$-stationary Nash equilibrium policy if for every 
$s\in S$,
$
\Phi(s, \pi^*) + \epsilon \geq \sup_{\pi \in \Pi} \Phi(s, \pi).
$
\end{proposition}




Proof of Proposition \ref{prop:approximate_eq} is provided in Appendix \ref{ssec: ProofPropApproximateEq}.

Proposition \ref{prop:approximate_eq}  indicates that when the \(\mnpg\)-potential function is known, any algorithm that computes the maximizer of the $\alpha$-potential function can be used to approximate stationary Nash equilibrium of the Markov \(\mnpg\)-potential game.
However, the 
\(\mnpg\)-potential function associated with a Markov \(\mnpg\)-potential game may not be unique and may be unknown. Furthermore, the approach of approximating equilibrium by maximizing \(\mnpg\)-equilibrium is not amenable to online learning. Therefore, in Section \ref{sec: Algorithms}, we present two algorithms which do not require knowledge of \(\mnpg\)-potential functions and can be implemented in an online manner.
}
\end{comment}

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Markov $\alpha$-Potential Games: Equilibrium Approximation and Regret Analysis}{X. Guo, X. Li, C. Maheshwari, S. Sastry, M. Wu}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Markov $\mnpg$-Potential Games: Equilibrium Approximation and Regret Analysis\thanks{Submitted to the editors DATE.}}

% Authors: full names plus addresses.
\author{Xin Guo\thanks{IEOR, UC Berkeley, CA
  (\email{xinguo@berkeley.edu}).}
\and Xinyu Li\thanks{IEOR, UC Berkeley, CA
  (\email{xinyu\_li@berkeley.edu}). (\textsf{Corresponding Author}).}
\and Chinmay Maheshwari\thanks{EECS, UC Berkeley, CA (\email{chinmay\_maheshwari@berkeley.edu}). (\textsf{Corresponding Author}).} \and Shankar Sastry\thanks{EECS, UC Berkeley, CA (\email{shankar\_sastry@berkeley.edu})} \and Manxi Wu\thanks{ORIE, Cornell University, NY (\email{manxiwu@cornell.edu})}}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

